Ion Coulomb Crystals in Storage Rings for Quantum Information Science

Quantum information science is a growing field that promises to take computing into a new age of higher performance and larger scale computing as well as being capable of solving problems classical computers are incapable of solving. The outstanding issue in practical quantum computing today is scaling up the system while maintaining interconnectivity of the qubits and low error rates in qubit operations to be able to implement error correction and fault-tolerant operations. Trapped ion qubits offer long coherence times that allow error correction. However, error correction algorithms require large numbers of qubits to work properly. We can potentially create many thousands (or more) of qubits with long coherence states in a storage ring. For example, a circular radio-frequency quadrupole, which acts as a large circular ion trap and could enable larger scale quantum computing. Such a Storage Ring Quantum Computer (SRQC) would be a scalable and fault tolerant quantum information system, composed of qubits with very long coherence lifetimes. With computing demands potentially outpacing the supply of high-performance systems, quantum computing could bring innovation and scientific advances to particle physics and other DOE supported programs. Increased support of R$\&$D in large scale ion trap quantum computers would allow the timely exploration of this exciting new scalable quantum computer. The R$\&$D program could start immediately at existing facilities and would include the design and construction of a prototype SRQC. We invite feedback from and collaboration with the particle physics and quantum information science communities.

==> workshopsymbols.tex <==
%%%%   Standard symbols for use in Snowmass Working Group Proceedings%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  basic formatting macros:%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%   text mode macros

\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\ibid{{\it ibid}.}

\def\Acknowledgements{\bigskip  \bigskip \begin{center} \begin{large}
             \bf ACKNOWLEDGEMENTS \end{large}\end{center}}


%  equation display macros
%https://www.overleaf.com/project/620e6f0016f3a4126579addc
\def\beq{\begin{equation}}
\def\eeq#1{\label{#1}\end{equation}}
\def\eeqn{\end{equation}}

%%  multiple-line equations  (use \CR as the carriage return):

\newenvironment{Eqnarray}%
   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
\def\beqa{\begin{Eqnarray}}
\def\eeqa#1{\label{#1}\end{Eqnarray}}
\def\eeqan{\end{Eqnarray}}
\def\CR{\nonumber \\ }

%%  reference to an equation number:

\def\leqn#1{(\ref{#1})}

%%  sizing and bars

\def\st{\scriptstyle}
\def\sst{\scriptscriptstyle}

\def\overbar#1{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar

\def\subscr#1{{\mbox{\scriptsize #1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  expectation values: 

\def\VEV#1{\left\langle{ #1} \right\rangle}
\def\bra#1{\left\langle{ #1} \right|}
\def\ket#1{\left| {#1} \right\rangle}
\def\vev#1{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% relation symbols

\def\lsim{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\gsim{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}

\def\Im{{\rm Im}}
\def\Re{{\rm Re}}
\def\tr{{ \rm tr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  caligraphic letters (for matrix elements, luminosity, etc.)

\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}
\def\H{{\cal H}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  matrix operations and fractions:

\def\One{{\bf 1}}
\def\hc{{\mbox{\rm h.c.}}}
\def\tr{{\mbox{\rm tr}}}
\def\half{\frac{1}{2}}
\def\thalf{\frac{3}{2}}
\def\third{\frac{1}{3}}
\def\tthird{\frac{2}{3}}

\def\del{\partial}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}
\def\pslash{\not{\hbox{\kern-2pt $p$}}}
\def\ETmiss{\not{\hbox{\kern-4pt $E$}}_T}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  high-energy physics terminology:

\def\Pl{{\mbox{\scriptsize Pl}}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\GUT{{\mbox{\scriptsize GUT}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\gw{\Gamma_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_H}
\def\gh{\Gamma_H}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\MSB{{\bar{M \kern -2pt S}}}
\def\msb{{\bar{\scriptsize M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\drb{{\bar{\scriptsize D \kern -1pt R}}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}
\def\Kzero{K^0}
\def\Kzerobar{{\bar K}^0}
\def\Dzero{D^0}
\def\Dzerobar{{\bar D}^0}
\def\Bzero{B^0}
\def\Bzerobar{{\bar B}^0}


%%%%%%%%%%%%   units for math mode  %%%%%%%%%%%%%%%%%%%%%%%%%

\def\ifb{{\rm fb}^{-1}}
\def\eV{{\rm eV}}
\def\keV{{\rm keV}}
\def\MeV{{\rm MeV}}
\def\GeV{{\rm GeV}}
\def\TeV{{\rm TeV}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  supersymmetry:

\def\ch#1{\widetilde\chi^+_{#1}}
\def\chm#1{\widetilde\chi^-_{#1}}
\def\neu#1{\widetilde\chi^0_{#1}}
\def\s#1{\widetilde{#1}}



%%%%%%%%%%  common journal names   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\aj{{Astronomical Journal}}%
\newcommand\araa{{Annual Review of Astron and Astrophys}}%
 \newcommand\apj{{Astrophysical Journal}}%
\newcommand\apjl{{Astrophysical Journal, Letters}}%
\newcommand\apjs{{ApJS}}%
% Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}%
% Applied Optics
\newcommand\apss{{Ap\&SS}}%
% Astrophysics and Space Science
\newcommand\aap{{Astronomy and Astrophysics}}%
\newcommand\aapr{{A\&A~Rev.}}%
% Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}%
% Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}%
% Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}%
% Bulletin of the AAS
\newcommand\jrasc{{JRASC}}%
% Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}%
% Memoirs of the RAS
\newcommand\mnras{{Monthly Notices of the Royal Astronomical Society}}%
\newcommand\pra{{Phys.~Rev.~A}}%
% Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}%
% Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}%
% Physical Review C
\newcommand\prd{{Physics~Review~D}}%
% Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}%
% Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}%
% Physical Review Letters
\newcommand\pasp{{Publications of the ASP}}%
\newcommand\pasj{{PASJ}}%
% Publications of the ASJ
\newcommand\qjras{{QJRAS}}%
% Quarterly Journal of the RAS
\newcommand\jcap{{JCAP}}%
\newcommand\skytel{{S\&T}}%
% Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}%
% Solar Physics
\newcommand\sovast{{Soviet~Ast.}}%
% Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}%
% Space Science Reviews
\newcommand\zap{{ZAp}}%
% Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}%
\newcommand\iaucirc{{IAU~Circ.}}%
% IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}}%
% Astrophysics Letters
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}%
% Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}%
% Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}%
% Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}%
% Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}}%
% Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}%
% Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}%
% Journal of Geophysics Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}%
% Journal of Quantitative Spectroscopy and Radiative Transfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}%
% Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}%
% Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}%
% Physics Reports
\newcommand\physscr{{Phys.~Scr}}%
% Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}%
% Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
